Fully 3D Unrolled Magnetic Resonance Fingerprinting Reconstruction via Staged Pretraining and Implicit Gridding

Magnetic Resonance Fingerprinting (MRF) enables fast quantitative imaging, yet reconstructing high-resolution 3D data remains computationally demanding. Non-Cartesian reconstructions require repeated non-uniform FFTs, and the commonly used Locally Low Rank (LLR) prior adds computational overhead and becomes insufficient at high accelerations. Learned 3D priors could address these limitations, but training them at scale is challenging due to memory and runtime demands. We propose SPUR-iG, a fully 3D deep unrolled subspace reconstruction framework that integrates efficient data consistency with a progressive training strategy. Data consistency leverages implicit GROG, which grids non-Cartesian data onto a Cartesian grid with an implicitly learned kernel, enabling FFT-based updates with minimal artifacts. Training proceeds in three stages: (1) pretraining a denoiser with extensive data augmentation, (2) greedy per-iteration unrolled training, and (3) final fine-tuning with gradient checkpointing. Together, these stages make large-scale 3D unrolled learning feasible within a reasonable compute budget. On a large in vivo dataset with retrospective undersampling, SPUR-iG improves subspace coefficient maps quality and quantitative accuracy at 1-mm isotropic resolution compared with LLR and a hybrid 2D/3D unrolled baseline. Whole-brain reconstructions complete in under 15-seconds, with up to $\times$111 speedup for 2-minute acquisitions. Notably, $T_1$ maps with our method from 30-second scans achieve accuracy on par with or exceeding LLR reconstructions from 2-minute scans. Overall, the framework improves both accuracy and speed in large-scale 3D MRF reconstruction, enabling efficient and reliable accelerated quantitative imaging.

==> shortcuts.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would not end up as ``with respect toblah''. 
\def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

% includes
\usepackage{amsmath, amssymb} 
\usepackage{amsmath}
\usepackage{bm}
\usepackage{xcolor}

\DeclareMathOperator{\Tr}{Tr}

\newcommand{\footnotestandalone}[1]{\let\thefootnote\relax\footnotetext{#1}}
\newcommand{\indicator}[1]{\mathbf{1}_{\{#1\}}}

% Numbers
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}

% colors
\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\bRED}[1]{{{\textbf{\RED{#1}}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}  
\newcommand{\bBLUE}[1]{{{\textbf{\BLUE{#1}}}}}  

\newcommand{\TBD}{\RED{[TBD]}}

\newcommand{\TODO}[1]{\RED{[TODO: #1]}}

% % Command abbreviations
\newcommand{\beite}{\begin{itemize}}
\newcommand{\enite}{\end{itemize}}
\newcommand{\beenu}{\begin{enumerate}}
\newcommand{\enenu}{\end{enumerate}}
\newcommand{\becen}{\begin{center}}
\newcommand{\encen}{\end{center}}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% \newcommand{\prox}{\text{prox}}
\newcommand{\prox}{{\mathrm{prox}}}
\newcommand{\minop}[1]{\ensuremath{\operatorname*{min}_{#1}}}
\newcommand{\maxop}[1]{\ensuremath{\operatorname*{max}_{#1}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}
\newcommand{\arginf}[1]{\ensuremath{\operatorname*{arg\,inf}_{#1}}}
\newcommand{\argsup}[1]{\ensuremath{\operatorname*{arg\,sup}_{#1}}}


\makeatletter
\newcommand*{\indep}{%
  \mathbin{%
    \mathpalette{\@indep}{}%
  }%
}
\newcommand*{\nindep}{%
  \mathbin{%                   % The final symbol is a binary math operator
    \mathpalette{\@indep}{\not}% \mathpalette helps for the adaptation
                               % of the symbol to the different math styles.
  }%
}
\newcommand*{\@indep}[2]{%
  % #1: math style
  % #2: empty or \not
  \sbox0{$#1\perp\m@th$}%        box 0 contains \perp symbol
  \sbox2{$#1=$}%                 box 2 for the height of =
  \sbox4{$#1\vcenter{}$}%        box 4 for the height of the math axis
  \rlap{\copy0}%                 first \perp
  \dimen@=\dimexpr\ht2-\ht4-.2pt\relax
      % The equals symbol is centered around the math axis.
      % The following equations are used to calculate the
      % right shift of the second \perp:
      % [1] ht(equals) - ht(math_axis) = line_width + 0.5 gap
      % [2] right_shift(second_perp) = line_width + gap
      % The line width is approximated by the default line width of 0.4pt
  \kern\dimen@
  {#2}%
      % {\not} in case of \nindep;
      % the braces convert the relational symbol \not to an ordinary
      % math object without additional horizontal spacing.
  \kern\dimen@
  \copy0 %                       second \perp
} 
\makeatother

\newcommand*{\nperp}{\not\perp}

% expectation
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}\mathrm{ar}}

% bolds
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bd}{{\bf d}}
\newcommand{\be}{{\bf e}}
\newcommand{\bdf}{{\bf f}}
\newcommand{\bg}{{\bf g}}
\newcommand{\bh}{{\bf h}}
\newcommand{\bi}{{\bf i}}
\newcommand{\bj}{{\bf j}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bl}{{\bf l}}
% \newcommand{\bm}{{\bf m}}
\newcommand{\bn}{{\bf n}}
\newcommand{\bo}{{\bf o}}
\newcommand{\bp}{{\bf p}}
\newcommand{\bq}{{\bf q}}
\newcommand{\br}{{\bf r}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bt}{{\bf t}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bz}{{\bf z}}
\newcommand{\beps}{{\boldsymbol{\epsilon}}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bG}{{\bf G}}
\newcommand{\bH}{{\bf H}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bJ}{{\bf J}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bL}{{\bf L}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bO}{{\bf O}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bQ}{{\bf Q}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bW}{{\bf W}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bZ}{{\bf Z}}

% bold greek
\newcommand{\balpha}{{\bm{\alpha}}}
\newcommand{\bbeta}{{\bm{\beta}}}
\newcommand{\bgamma}{{\bm{\gamma}}}
\newcommand{\bdelta}{{\bm{\delta}}}
\newcommand{\bepsilon}{{\bm{\epsilon}}}
\newcommand{\bzeta}{{\bm{\zeta}}}
\newcommand{\btheta}{{\bm{\theta}}}
\newcommand{\biota}{{\bm{\iota}}}
\newcommand{\bkappa}{{\bm{\kappa}}}
\newcommand{\blambda}{{\bm{\lambda}}}
\newcommand{\bmu}{{\bm{\mu}}}
\newcommand{\bnu}{{\bm{\nu}}}
\newcommand{\bxi}{{\bm{\xi}}}
\newcommand{\bomicron}{{\bm{\omicron}}}
\newcommand{\bpi}{{\bm{\pi}}}
\newcommand{\brho}{{\bm{\rho}}}
\newcommand{\bsigma}{{\bm{\sigma}}}
\newcommand{\btau}{{\bm{\tau}}}
\newcommand{\bupsilon}{{\bm{\upsilon}}}
\newcommand{\bphi}{{\bm{\phi}}}
\newcommand{\bchi}{{\bm{\chi}}}
\newcommand{\bpsi}{{\bm{\psi}}}
\newcommand{\bomega}{{\bm{\omega}}}

\newcommand{\bGamma}{{\bm{\Gamma}}}
\newcommand{\bDelta}{{\bm{\Delta}}}
\newcommand{\bTheta}{{\bm{\Theta}}}
\newcommand{\bLambda}{{\bm{\Lambda}}}
\newcommand{\bXi}{{\bm{\Xi}}}
\newcommand{\bPi}{{\bm{\Pi}}}
\newcommand{\bSigma}{{\bm{\Sigma}}}
\newcommand{\bUpsilon}{{\bm{\Upsilon}}}
\newcommand{\bPhi}{{\bm{\Phi}}}
\newcommand{\bPsi}{{\bm{\Psi}}}
\newcommand{\bOmega}{{\bm{\Omega}}}

% calligraphy
\newcommand{\cA}{{\cal A}}
\newcommand{\bcA}{{\bf \cal A}}
\newcommand{\bcP}{{\bf \cal P}}
\newcommand{\bcD}{{\bf \cal D}}
\newcommand{\bcE}{{\bf \cal E}}
\newcommand{\bcF}{{\bf \cal F}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}

\newcommand{\bone}{{\bf 1}}
\newcommand{\bzr}{{\bf 0}}


% Norm
\newcommand{\ellOne}{\ensuremath{{\ell_1}}}
\newcommand{\ellTwo}{\ensuremath{{\ell_2}}}
\newcommand{\ellp}{\ensuremath{{\ell_p}}}
\newcommand{\ellInfty}{\ensuremath{{\ell_\infty}}}

% It is better not to use ensuremath for these norms, as they would look funny when, e.g., they are squared.
\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\ellOneNorm}[1]{{\norm{#1}_{\ellOne}}}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellpNorm}[1]{{\norm{#1}_{\ellp}}}
\newcommand{\ellInftyNorm}[1]{{\norm{#1}_{\ellInfty}}}
\newcommand{\Fnorm}[1]{\left\|{#1}\right\|_F}

\newcommand{\ellTwoDist}[2]{d(#1,#2)_\ellTwo}
\newcommand{\ellOneDist}[2]{d(#1,#2)_\ellOne}
\newcommand{\SigmaDist}[2]{d(#1,#2)_\Sigma}

\newcommand{\Fdist}[2]{{d(#1,#2)_F}}

\newcommand{\DistExt}[2]{{d(#1,#2)_{\mathrm{Ext}}}}

\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\SOthree}{\mathrm{SO}(3)}
\newcommand{\sothree}{\mathfrak{so}(3)}

\newcommand{\SE}[1]{\ensuremath{\mathrm{SE(#1)}}}
\newcommand{\se}[1]{\ensuremath{\mathrm{se(#1)}}}

\newcommand{\GL}[1]{\ensuremath{\mathrm{GL(#1)}}}
\newcommand{\gl}[1]{\ensuremath{\mathrm{gl(#1)}}}
\newcommand{\GLn}{\GL{n}}
\newcommand{\GLthree}{\GL{3}}

\newcommand{\tp}{t_p}
\newcommand{\nopt}{n_{\rm{opt}}}

\newcommand{\GLnPlus}{\ensuremath{\mathrm{GL_{+}(n)}}}

\newcommand{\gln}{\ensuremath{\mathfrak{gl}(n)}}


\newcommand{\FRAME}[2]{
\begin{frame}
\begin{frametitle}{#1}
\end{frametitle}
#2
\end{frame}}

\newcommand{\BLOCK}[2]{
\begin{block}{#1}
#2
\end{block}}

\newcommand{\Ncols}{{N_{\text{cols}}}}
\newcommand{\Nrows}{{N_{\text{rows}}}}

\newcommand{\Nedges}{{N_{\text{edges}}}}


\newcommand\comment[1]{\textcolor{red}{#1}}

% dataset
\newcommand{\Dataset}{\mathfrak{D}}
\newcommand{\Validation}{\mathfrak{D}_v}

% fig captioning
%\usepackage[justification=centering]{caption}
%\usepackage{subcaption}

\newcommand{\DiffusionStep}{\operatorname{Diffusion-Step}}
\newcommand{\DDIMStep}{\operatorname{DDIM-Step}}
\newcommand{\CG}{\operatorname{CG-SENSE}}
\newcommand{\xinit}{\bx_{\rm{init}}}
\newcommand{\zinit}{\bz_{\rm{init}}}
\newcommand{\xside}{\bx_s}
\newcommand{\xgt}{\bx^\star}
\newcommand{\zgt}{\bz^\star}
\newcommand{\balph}{\bar{\alpha}_t}
\newcommand{\xp}{\bx^{\text{P}}}
\newcommand{\zp}{\bz^{\rm{P}}}
\newcommand{\ntr}{N_{\text{TR}}}

\newcommand{\abart}{\bar \alpha_t}
\newcommand{\tpemp}{t_p^{\star, \rm{obs}}}
\newcommand{\tpapprox}{{\tilde t}_{p}}

\newcommand{\tpscale}{v_{\rm{p}}}
\newcommand{\tpshift}{w_{\rm{p}}}

\newcommand{\tprev}{t_{\rm{prev}}}
\newcommand{\zprev}{\bz_{\rm{prev}}}
\newcommand{\tstep}{\Delta t}
\newcommand{\nstep}{n_{\rm{step}}}
\newcommand{\navg}{n_{\rm{avg}}}
\newcommand{\mineq}{-=}

\newcommand\bitsmall{\fontsize{9}{11}\selectfont}


